Meta-Embedding as Auxiliary Task Regularization

Word embeddings have been shown to benefit from ensambling several word embedding sources, often carried out using straightforward mathematical operations over the set of word vectors. More recently, self-supervised learning has been used to find a lower-dimensional representation, similar in size to the individual word embeddings within the ensemble. However, these methods do not use the available manually labeled datasets that are often used solely for the purpose of evaluation. We propose to reconstruct an ensemble of word embeddings as an auxiliary task that regularises a main task while both tasks share the learned meta-embedding layer. We carry out intrinsic evaluation (6 word similarity datasets and 3 analogy datasets) and extrinsic evaluation (4 downstream tasks). For intrinsic task evaluation, supervision comes from various labeled word similarity datasets. Our experimental results show that the performance is improved for all word similarity datasets when compared to self-supervised learning methods with a mean increase of $11.33$ in Spearman correlation. Specifically, the proposed method shows the best performance in 4 out of 6 of word similarity datasets when using a cosine reconstruction loss and Brier's word similarity loss. Moreover, improvements are also made when performing word meta-embedding reconstruction in sequence tagging and sentence meta-embedding for sentence classification.

==> notes/analogy_notes.tex <==
\iffalse
It would be somewhat unsurprising that the embeddings do not outperform single embeddings since not all the algorithms are known to preserve analogical relations. 
We propose to create a dataset in which word pairs are manually classified into various categories, as in past SemEval tasks, but furthermore word pairs within a category are manually distinguished according to how well they represent the category; that is, the degree to which they are relationally similar to prototypical members of the given semantic relation class. This dataset will be used in two tasks.

Dataset used in competition was scored as in golden scoring (which scoring) parameter, however organiser have release improved labels afterwards (platinium scoring) The task is, given two pairs of words, $(A:B)$ and $(C:D)$, determine the degree to which the semantic relations between A and B are similar to those between C and D. Unlike the more familiar task of semantic relation identification, which assigns each word pair to a discrete semantic relation class, this task recognizes the continuous range of  degrees of relational similarity. The challenge is to determine the degrees of relational similarity between a given reference word pair and a variety of other pairs, mostly in the same general semantic relation class as the reference pair.
\fi


\iffalse
Curating guidelines for manual annotations of different analogy relation types can be complex to construct and follow. 
In this case the architecture takes on a slight variation that allows for learning the relationship between pairs of word pairs, as is the case in analogy tasks. We can instead pass input analogy pairs $(x_1^{1}, x_2^{1})$ and $(x_1^{2}, x_2^{2})$ and predict if they are analogous or not. Alternatively, we can take $(x_1^{1}, x_2^{1})$ and $x_1^{2}$ so to predict $x_2^{2}$ and vice-versa. In the latter case, the output is high dimensional and a more difficult than the former. Furthermore, we can learn to also predict the type of part-of-speech category for analogy pair for supervision.  

The analogy reconstruction $\mathcal{L}_{r}^{a}$ is then shown in Equation \ref{eq:analogy_recon} which minimizes the $\ell_2$ between pairwise difference (PairDiff).

\begin{equation}\label{eq:analogy_recon}
\begin{split}
	\mathcal{L}^{a}_{r} = \sum_{i=1}^{N}\Big[\Big((x_{(i,1)}^{1} + x_{(i,2)}^{1}) - (\hat{x}_{(i, 1)}^{1} +  \hat{x}_{(i,2)}^{1})\Big)^{2} + \\
 \Big((x_{(i,1)}^{2} + x_{(i,2)}^{2}) - (\hat{x}_{(i, 1)}^{2} + \hat{x}_{(i,2)}^{2})\Big)^{2} \Big]
\end{split}
\end{equation}

We also learn to predict the PoS of the analogical relation in a multi-label classification as apart of the branch of the network (i.e $h^{2}-h^{3}$). We can do so by using a sigmoid output for all possible (nn, nns, nnpos, jj,   jjs, jjr, vb, vbd, vbz) PoS and choosing the two most probable outputs, since we know there must be only two. That is to point out, we do not use the commonly used thresholding of the sigmoid but rather an $argmax$. However, this treats the labels as independent, therefore we also experiment with choosing the top 2 probabilities of from $\mathtt{softmax}$, $\phi$.

The reason for posing this as multi-class bi-label classification is because if we treated the PoS pair as a single label (e.g jj-jjr), all misclassifications are considered equal. Therefore, getting one of the two pairs correct would be the same as misclassifying both which we want to avoid. By learning to predict PoS relation type given encoded analogy pairs we encourage the model to learn \textbf{IS THIS RUBBISH ?}

\begin{equation}\label{eq:analogy_pos_out}
%\begin{split}
%\mathcal{L}_{a} = \hat{y}^{2}_{(i, 2)}  \\
\hat{y} = \phi \Bigg(\Big(h_{1}^{(l,1)} \oplus h_{2}^{(l,1)}\Big) -   \Big(h_{1}^{(l,2)} \oplus h_{2}^{(l,2)}\Big) \Bigg)
%\end{split}
\end{equation}

\fi

==> notes/other_tasks.tex <==
\iffalse Chunking\fi and Sentiment Analysis (SA) as three extrinsic tasks. 
\iffalse
\DB{Is sentiment analysis a structure prediction task? It is more like a text classification task. Perhaps we can remove the bit ``more specifically structured predictions problems.'' from that sentence?}
\fi

